Position Paper: From Multi-Agent Pathfinding to Pipe Routing

The 2D Multi-Agent Path Finding (MAPF) problem aims at finding collision-free paths for a number of agents, from a set of start locations to a set of goal positions in a known 2D environment. MAPF has been studied in theoretical computer science, robotics, and artificial intelligence over several decades, due to its importance for robot navigation. It is currently experiencing significant scientific progress due to its relevance in automated warehousing (such as those operated by Amazon) and in other contemporary application areas. In this paper, we demonstrate that many recently developed MAPF algorithms apply more broadly than currently believed in the MAPF research community. In particular, we describe the 3D Pipe Routing (PR) problem, which aims at placing collision-free pipes from given start locations to given goal locations in a known 3D environment. The MAPF and PR problems are similar: a solution to a MAPF instance is a set of blocked cells in x-y-t space, while a solution to the corresponding PR instance is a set of blocked cells in x-y-z space. We show how to use this similarity to apply several recently developed MAPF algorithms to the PR problem, and discuss their performance on abstract PR instances. We also discuss further research necessary to tackle real-world pipe-routing instances of interest to industry today. This opens up a new direction of industrial relevance for the MAPF research community.

==> Makefile <==
FICHIER = socs19

TEXFILES = $(wildcard *.tex) $(wildcard images/*.tex) $(wildcard algo/*.tex) $(wildcard tikz/*.tex) 
BIBFILE  = $(wildcard *.bib)
FIGFILES = $(wildcard images/*.fig)
EPSFILES = $(patsubst %.fig,%.eps,$(FIGFILES))

TMPFILES  = $(wildcard *.aux) $(wildcard *.bbl) $(wildcard *.ps) $(wildcard *.dvi) $(wildcard *.blg) $(wildcard *.toc) $(wildcard *.lof) $(wildcard *.log) $(wildcard *.lot) 
BACKFILES = $(wildcard *.bak) $(wildcard */*.bak) $(wildcard *~) $(wildcard */*~) $(wildcard *.tar.gz)
TRUCFILES = $(wildcard _*)

DOTFILES = $(wildcard *.dot)
PSDOTFILES = $(patsubst %.dot,%.tps,$(DOTFILES))

all: $(FICHIER).pdf

%.pdf: $(TEXFILES)
	pdflatex $(FICHIER)
	if grep -q 'citation' $(FICHIER).aux; then if grep -q 'bibdata' $(FICHIER).aux; then bibtex $(FICHIER); fi else rm -f $(FICHIER).bbl; fi
	pdflatex $(FICHIER) 
	pdflatex $(FICHIER)

#%.pdf: %.ps
#	ps2pdf $<

#%.tps: %.dot
#	dot -Tps -o $@ $<

%.ps:  %.dvi
	dvips -o $@ $< > /dev/null
#	dvips -Pcmz -Pamz -o $@ $< > /dev/null

%.eps: %.fig
	fig2dev -L eps $< $@

%.dvi: _tpsfiles _epsfiles $(TEXFILES)
	pdflatex $(FICHIER)
	if grep -q 'citation' $(FICHIER).aux; then if grep -q 'bibdata' $(FICHIER).aux; then bibtex $(FICHIER); fi else rm -f $(FICHIER).bbl; fi
	pdflatex $(FICHIER) > /dev/null
	pdflatex $(FICHIER) > /dev/null

_tpsfiles: $(PSDOTFILES)
	touch _tpsfiles

%.tps: %.dot
	dot -Tps -o $@ $<

_epsfiles: $(EPSFILES)
	@echo $(EPSFILES) > _epsfiles

clean:
	-rm -f $(EPSFILES) $(BACKFILES) $(PSDOTFILES)
	-rm -f $(TMPFILES)
	-rm -f $(TRUCFILES)
	-rm -f $(FICHIER).pdf

tar: clean
	perl -e '$$line=`date +"\%y-\%m-\%d"`;chomp($$line);`tar cvf $(FICHIER)-$$line.tar *`;`gzip $(FICHIER)-$$line.tar`;';

tardir: clean
	perl -e '$$pwd = `pwd`; my($$path,$$dir) = $$pwd =~ m/(.*\/)(.*)$$/; $$line=`date +"\%y-\%m-\%d"`;chomp($$line);`cd .. ; tar cvf $$dir-$$line.tar $$dir ; gzip $$dir-$$line.tar ; mv $$dir-$$line.tar.gz $$dir`;';

pwd:
	perl -e '$$pwd = `pwd`; print $$pwd;'

touch:
	@touch $(FICHIER).tex
	@echo You touch my ``$(FICHIER)''.

open:
#	@kile $(FICHIER).tex &
#	@texmaker $(FICHIER).tex &
	@emacs $(FICHIER).tex &





==> alg_pbs.tex <==
begin{algorithm}
\caption{High-Level Search of PBS}\label{euclid}
\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
\Input{Environment files, start locations and goal locations of synthetic instances}
\Output{Paths}
$\prec_{Root} \gets \prec_{\emptyset}$ \;
$Root.plan \gets \emptyset$ \;
\For{each $i \in [M]$}
{
$success \gets GetPlan(Root, a_{i})$ \;
\If{$\lnot success$}
{\Return "No Solution" \;}
}
$Root.cost \gets$ sum of the lengths in $Root.plan$ \;
$\STACK \gets$ $\{Root\}$ \;
\While{$\STACK \neq \emptyset$}
{
$N \gets$ top node in \STACK \;
$\STACK \gets \STACK \setminus \{N\}$ \;
\If{$N.plan$ does not have any collision}
{\Return $N.plan$ \;}
$C \gets$ the first collision $<a_i, a_j>$ in $N.plan$ \;
\For{each $a_i$ involved in $C$}
{
$N^{'} \gets$ new node \;
$N^{'}.plan \gets N.plan$ \;
$\prec_{N^{'}} \gets \prec_{N} \cup \{j \prec i\}$ \;
$success \prec GetPlan(N^{'}, a_i)$ \;
\If{$success$}
{$N^{'}.cost \gets$ sum of the lengths in $N^{'}.plan$ \;}
}
$\STACK \gets \STACK \cup \{N^{'}\}$ \;
}
\Return "No Solution" \;
\end{algorithm}

